Gaseous argon time projection chamber with electroluminescence enhanced optical readout

Systematic uncertainties in accelerator oscillation neutrino experiments arise mostly from nuclear models describing neutrino-nucleus interactions. To mitigate these uncertainties, we can study neutrino-nuclei interactions with detectors possessing enhanced hadron detection capabilities at energies below the nuclear Fermi level. Gaseous detectors not only lower the particle detection threshold but also enable the investigation of nuclear effects on various nuclei by allowing for changes in the gas composition. This approach provides valuable insights into the modelling of neutrino-nucleus interactions and significantly reduces associated uncertainties. Here, we discuss the design and first operation of a gaseous argon time projection chamber optically read. The detector operates at atmospheric pressure and features a single stage of electron amplification based on a thick GEM. Here, photons are produced with wavelengths in the vacuum ultraviolet regime. In an optical detector the primary constraint is the light yield. This study explores the possibility of increasing the light yield by applying a low electric field downstream of the ThGEM. In this region, called the electroluminescence gap, electrons propagate and excite the argon atoms, leading to the subsequent emission of photons. This process occurs without any further electron amplification, and it is demonstrated that the total light yield increases up to three times by applying moderate electric fields of the order of 3~kV/cm. Finally, an indirect method is discussed for determining the photon yield per charge gain of a ThGEM, giving a value of 18.3 photons detected per secondary electron.

==> Sections/1Introduction.tex <==
% \textcolor{orange}{CS: A few inconsistencies that I found throughout the paper and that would be easy to clean up:
% \begin{itemize}
%     \item \textcolor{teal}{ "Argon" should appear with lower case unless it starts a sentence}
%     \item spaces between numbers and units (maybe use the siunitx package) \textcolor{teal}{between number and unit there should be a little space made by putting ~ in between.lke here : 10~cm. Does this make sense? I am gonna adjust all}
%     \item sometimes element symbols are in italics \textcolor{teal}{I think I fixed it all}
%     \item spaces before acronyms in parentheses, e.g. ultra-violet(UV), visible light (VL)
%     \textcolor{teal}{here we should stick to space between}
%     \item spaces after approx, e.g. $\approx$50\% (also maybe "$\sim$" is better in many places but this might be a personal preference)
%     \item you often mention RMS in the signal definition. Technically, there is a difference between RMS and standard deviation and I think you mean the latter. But these are often used interchangeably
%     \item waveform / wave-form
% \end{itemize}
% }


\section{Introduction}

Many physics experiments require the reconstruction of all charged particle tracks leaving the interaction vertex and also the ability to
identify by statistical means the particle types produced in the physics process. Detectors which provide this information are called {\it trackers}. Depending on the experimental environment, either solid-state, scintillating or gaseous detectors are
used. In environments where large areas need to be covered cost-effectively and with a low material budget, the latter is the optimal choice. Examples of gaseous detectors include  Geiger counters, straw tubes, multi-wire proportional chambers and time projection chambers (TPC). 

The concept of a TPC was invented in the late 1970s by D. Nygren \cite{Nygren:1980ue}. \textcolor{red}{[LG]A TPC consists of a volume filled with a suitable gas, and a cathode and an anode on opposite sides of the volume. By applying a negative high voltage (HV) to the cathode while keeping the anode at ground or a moderate positive voltage, an electric field, the so-called {\it drift field} is created. To achieve a very homogeneous drift field, metallic strips are placed on the walls and connected via suitable resistors, to the cathode on one side and to ground on the other side. With these strips,  called field strips, the electric potential is well defined at every position between the two electrodes. As fill gas, in general a noble gas is used, typically argon mixed with a certain percentage of other molecular gases such as CH4, iC4H10 or CF4. The choice of the gas mixture
significantly affects the detector's performance. The basic working principle of a TPC is that a charged particle traversing the gas ionises it, releasing in the process electron-ion pairs. The ions slowly drift towards the cathode where
they normally are absorbed undetected. The electrons, on the other hand, drift towards the anode. The anode is segmented into 
small pads, allowing track reconstruction on the projected xy plane. Knowing the time when the interaction has happened, either by exploiting a fast trigger signal from an outer scintillator plane or from the accelerator, the position along the drift direction (z-direction) can also be reconstructed. In this way, a full 3D 
event reconstruction can be achieved.} \\
\textcolor{green}{[LG]A TPC consist of a gas filled volume where an homogeneous and uniform electric field is applied, enclosed by a field cage, a cathode and a segmented anode. The TPC allows 3D tracking by reconstructing the projected track on the anode plane and using the time information of electrons reaching the anode from the ionisation point.
As fill gas, in general a noble gas is used, typically argon mixed with a certain percentage of other molecular gases such as CH4, iC4H10 or CF4. The choice of the gas mixture
significantly affects the detector's performance.}
A problem with this approach is that a minimal ionising particle only produces around 90 electrons per cm in argon, not enough to be detected directly. For this reason, an amplification stage is installed directly in front of the anode. The amplification stage consists of a region in which a very high electric field is created. An electron released in the drift volume which enters this region undergoes a charge avalanche process in which between hundreds and a few thousand electron-ion pairs are created. The signal (charge) amplified in this way is sufficient to be detected with cost-effective electronics. \textcolor{red}{[LG]The ions, also produced in this avalanche, have the tendency to drift towards the cathode if not absorbed earlier. This is a potential problem in high-rate environments
since the large concentration of positive ions might change the drift field locally.} For the amplification stage,
several technologies are available: wires, MicroMegas (MM), Gas Electron Multipliers (GEMs) and Thick GEMs (ThGEM), also called Large Electron Multipliers (LEMs), for example.\\
The described concept was and is used successfully in a wide range of experiments, including the heavy ion experiment ALICE and the neutrino experiment T2K. However, in some cases, this classical approach cannot be implemented for various reasons and alternative ideas based on an optical readout must be explored.  

An optical TPC is based on the same concept as the previously discussed one, with the fundamental difference that the particle detection happens not by the means of charge, but through the photons produced during the avalanche multiplication process. Every time an electron excites a gas atom, in the de-excitation process, photons are emitted; in the case of pure argon they have a wavelength in the Vacuum Ultraviolet (VUV) range, peaking at 128 nm. Placing a suitable optical system to detect these photons allows reconstructing of the event as with a charge readout. 


One of the main draw-backs of optical TPCs is that only a small fraction of the total photons produced reach the detection plane. This happens mainly due to the poor geometrical acceptance of the photons which are emitted at uniform angles. This effect is studied in depth for TPC based on pure argon gas, such as ~\cite{Monteiro:2008zz} or~\cite{ArgonLight:BUZULUTSKOV}. In the present paper, a similar TPC, based on based on pure argon gas at atmospheric pressure is studied, with the difference that the light production is based on two stages. Firstly, a ThGEM kept at a constant electric field is used, where electrons undergo avalanche multiplication. The ThGEM is followed by a mesh, space in which an additional low electric field is placed. In this space, named the electroluminescence (EL) gap, electron created in the ThGEM propagate further and they produce  



\textcolor{teal}{One of the main draw-backs of optical TPCs is that only a small fraction of the produced photons can be detected. This occurs mainly due to the geometrical acceptance of the photons within the TPC, but also due to various quantum efficiencies within the system. If not enough photons are produced, then the detection overall is affected, leading to a high amount of ionisation needed for particle detection. Papers such as~\cite{Monteiro:2008zz} or~\cite{ArgonLight:BUZULUTSKOV}, show an in depth study of the light yield of a pure argon TPC,  produced with a ThGEM or several GEMs chained together. }


Additionally, the light yield is increased using an additional region of electric field, where electrons excite the argon atoms, but do not ionise them. 




In this case, the motivation for this R\&D is the possible study of neutrino interaction cross sections in the context of long-baseline neutrino oscillation experiments as T2K~\cite{T2K}, NOvA~\cite{nova}, Hyper-Kamiokande~\cite{Hyper-KamiokandeWorkingGroup:2014czz} and LBNF/DUNE~\cite{DUNE:2016hlj}. 


When a neutrino of several hundred to a few GeV interacts via charged current exchange with the detector medium, a lepton is created in the process. However, besides this leptonic system, which can be easily detected, hadrons of low energy may also be produced. To detect these with a very low energy threshold is a challenge. One possibility is to use a high-pressure TPC (HPTPC) filled with pure argon. In this case, the TPC gas itself acts as the target for the neutrinos. To increase the probability of interaction the operation of the TPC at a pressure of several bar to about 10 bar is desirable. In addition, to measure precisely the neutrino cross section on argon, the amount of gas mixture additives must be below 1\% in mass. \textcolor{red}{[LG]Both motivate the usage of an optical readout for this
application. \\}
\textcolor{green}{[LG]Optical read out offers the possibility to place the read out system on the outside of the drift volume, in a concept where a light-transparent window transfers the light information to the external read out device (possibly using an external lens system). This concept is advantageous for high pressure TPCs since the read out system does not have to suffer high pressure. On the other hand it can favour high purity systems considering that it is much easier to design a leakage-free gas volume when it does not have to include the read out system itself, but only a glass window.}


The article is structured as follows: In section \ref{sec:ExperimentalSetup} a complete description of the experimental set-up is given, continued in section \ref{Sec:LightProduction} with a description of the light production within the detector.  section \ref{sec:DataProc} describes the data pre-processing and the calibration of the photon detector, section \ref{sec:Results} focuses on the results and finally, the paper concludes with section \ref{sec:Concl}. 




% With their invention in the late 1970s \cite{Nygren:1980ue} Time Projection Chambers (TPCs) only grew in size and sophistication, nowadays being  key detectors in many experiments such as XENONnT~\cite{XENON}, T2K~\cite{T2K} or DUNE



% With their invention in the late 1970s\cite{Nygren:1980ue} time projection chambers (TPCs) quickly became popular tracking detectors, appearing in several high energy experiments such as  PEP-4 at SLAC, ALEPH and DELPHI at LEP. Since then, TPCs have grown in size and sophistication and now form the basis for liquid argon (LAr) \textcolor{orange}{CS: maybe quote DUNE as the largest LAr TPC} or xenon (LXe) detectors such as XENONnT~\cite{XENON}. They are also an important component in the near detectors of T2K~\cite{T2K} \textcolor{orange}{CS: Specify that T2K is gas argon}. etc...

% A charged particle passing through a TPC produces electron-ion pairs. Under the influence of an electric field applied to the chamber, the electrons drift towards the amplification and readout electronics, where their drift times can be used for track reconstruction. Traditionally, the particle trajectory reconstruction is based on the electrical charge produced in electron multiplying devices \textcolor{orange}{CS: here the electric charge is   really produced by the through-going particle and then amplified in the electron multiplying devices} \textcolor{teal}{what would you add, I am not sure I understand} such as MICROMEGAS~\cite{Giomataris:1995fq}, Gas Electron Multipliers (GEM)~\cite{Sauli:1997qp} or Thick GEMs (ThGEM)~\cite{Chechik:2004wq}. In this stage, together with electrical charge, it has been shown that large quantities of photons are produced. This opened the road for the so-called optical TPCs, in which the ionisation reconstruction is based only on photon detection, and for hybrid detectors, where the charge collection is used together with the photons. 

% With the development of both electronics and photon detection devices (notably the ones based on silicon), optical TPCs gained more popularity, even being considered as suitable replacements for their charge-readout counterparts. One key advantage of such detectors is that the read-out can be completely isolated from the active region and therefore this is not influenced by high pressure environments. Also, using a lens system, in optical TPCs large areas of the detector can be projected onto smaller size photon sensors. This has a direct impact on the building costs of detectors and therefore it is of great importance for producing particle detectors in a more efficient and sustainable way. 

% Many experiments today rely on LAr or dual-phase liquid and gaseous argon TPCs. Despite its recent successes~\cite{Roberts:2018sww}, the LAr TPC comes with a disadvantage: compared to gas, in a liquid environment the particle detection momentum threshold is  higher. This threshold is a potential handicap to, for example, neutrino experiments, where one major source of uncertainties comes from final state interactions. A neutrino interacting with a nucleus might result in two or more nucleons being emitted~\cite{Alexis}; the first nucleon might be above the threshold of a LAr TPC but the second most likely will be well below. 

% For these reasons, we explore in this letter the potential of an optical TPC based on pure gaseous argon. In such a detector, the amount of ionisation electrons produced by a particle crossing the detector will be lower than in a LAr detector, and therefore a smaller light yield is expected. In order to compensate for this, it is common that several GEMs or even ThGEMs are used; In this paper we propose and demonstrate the feasability of a TPC based on a single ThGEM, used in combination with a mesh. Emphasis is put on the latter, as it provides an additional stage of light amplification, through the process of electroluminescence (EL). 



==> Sections/notes_for_writing.tex <==



Acronyms usage:

Define acronyms but don't use the \ac{} syntax in the \section{} or subsection{}. If you use the \ac in the table of content, then the title of the section will directly have the acronym instead of the full name. 


==> acro_list.tex <==
\begin{acronym}[MPC] % Give the longest label here so that the list is nicely aligned
\acro{MWPC}{Multi Wire Proportional Chamber}
\acro{TLA}{Three Letter Acronym}
\acro{MSGC}{Micro-Strip Gas Counter}
\acro{GEM}{gaseous electron multiplier}
\acro{ThGEM}{thick gaseous electron multiplier}
\acro{PMT}{photo-multiplier tube}
\acro{Ar}{Argon}
\acro{LAr}{liquid argon}
\acro{GAr}{gaseous argon}
\acro{TPC}{time projection chamber}
\acro{VUV}{vacuum ultra violet}
\acro{UV}{ultra violet}
\acro{VL}{visible light}
\acro{IR}{infra red}
\acro{NB}{neutral brehmstrahlung}
\acro{EL}{electroluminescence}
\acro{WLS}{wavelength shifter}
\acro{PEN}{polyethylene naphthalate}
\acro{LFS}{last field stripe}

\end{acronym}
